Certainty Equivalence is Efficient for Linear Quadratic Control

We study the performance of the certainty equivalent controller on Linear Quadratic (LQ) control problems with unknown transition dynamics. We show that for both the fully and partially observed settings, the sub-optimality gap between the cost incurred by playing the certainty equivalent controller on the true system and the cost incurred by using the optimal LQ controller enjoys a fast statistical rate, scaling as the square of the parameter error. To the best of our knowledge, our result is the first sub-optimality guarantee in the partially observed Linear Quadratic Gaussian (LQG) setting. Furthermore, in the fully observed Linear Quadratic Regulator (LQR), our result improves upon recent work by Dean et al. (2017), who present an algorithm achieving a sub-optimality gap linear in the parameter error. A key part of our analysis relies on perturbation bounds for discrete Riccati equations. We provide two new perturbation bounds, one that expands on an existing result from Konstantinov et al. (1993), and another based on a new elementary proof strategy.

==> perturbation_dare.tex <==

\section{Perturbation of the discrete Riccati equation}
\label{sec:perturb}

In this section we upper bound the change in the solution to the Riccati equation when the system parameters are perturbed, based on a proof developed by \citet{konstantinov1993perturbation}. Compared to Theorem 3.2 of  \citet{konstantinov1993perturbation} we provide an interpretable result which has a linear dependence on the size of the parameter  perturbation.


We turn to the proof of this result. Given system parameters $(A,B)$ we denote by $F(X, A, B)$ the matrix expression
\begin{align}
  \label{eq:riccati_op}
  F(X, A, B) &= X - A^\top X A + A^\top X B (R + B^\top X B)^{-1} B^\top X A - Q\\
             &= X - A^\top X\left( I + B R^{-1} B^\top X  \right)^{-1}A - Q
               \label{eq:riccati_op_short}
\end{align}
Then, solving the Riccati equation associated to the system $(A,B)$ corresponds to finding the unique positive definite matrix $X$ such that $F(X, A, B) = 0$. We denote by $\Pstar$ the solution of the Riccati equation corresponding to the trye system parameters $(\Astar, \Bstar)$ and we denote by $\Phat$ the solution associated with the estimated dynamics $(\Ahat, \Bhat)$. Our goal is to upper bound $\norm{\Phat - \Pstar}$ in terms of $\varepsilon$, where $\varepsilon > 0$ such that $\norm{\Ahat - \Astar} \leq \varepsilon$ and $\norm{\Bhat - \Bstar} \leq \varepsilon$.

We denote $\Delta_P = \Phat - \Pstar$. The proof strategy goes as follows. Given the identities $F(\Pstar, \Astar, \Bstar) = 0$ and $F(\Phat, \Ahat, \Bhat) = 0$ we construct an operator $\opPhi$ such that $\Delta_P$ is its unique fixed point. Then, we show that the fixed point of $\opPhi$ must have small norm when $\varepsilon$ is sufficiently small.

We denote $S_\star = \Bstar R^{-1} \Bstar^\top$ and $\Shat = \Bhat R^{-1} \Bhat^\top$. For any matrix $X$ such that $I + \Sstar(\Pstar + X)$ is invertible we have
\begin{align}
  \label{eq:magical}
F(\Pstar + X, \Astar, \Bstar) &= X - L_\star^\top X L_\star + L_\star^\top X \left[I + S_\star (\Pstar + X)\right]^{-1} S_\star X L_\star.
\end{align}
To check this identity one needs to add  $F(\Pstar, \Astar, \Bstar)$, which is equal to zero, to the right hand side of \eqref{eq:magical} and use Lemma~\ref{lem:closed_loop_rewritten}, included in Appendix \ref{app:other}. To write \eqref{eq:magical} more compactly we define the following two matrix operators
\begin{align*}
\opT(X) = X - L_\star^\top X L_\star \;\text{ and }\; \opH(X) = L_\star^\top X \left(I + S_\star(\Pstar + X)\right)^{-1} S_\star X L_\star.
\end{align*}
Then, Equation~\ref{eq:magical} becomes $F(\Pstar + X, \Astar, \Bstar) = \opT(X) + \opH(X)$.
Since Equation~\ref{eq:magical} is satisfied by any matrix $X$ \propchange{with $I + S_\star(\Pstar+X)$}, the matrix equation
\begin{align}
  \label{eq:fixed_point_eq}
  F(\Pstar + X, \Astar, \Bstar) - F(\Pstar + X, \Ahat, \Bhat) = \opT(X) + \opH(X)
\end{align}
 has a unique symmetric solution $X$ such that $\Pstar + X \succeq 0$.
That solution is $X = \Delta_P$ because any solution of \eqref{eq:fixed_point_eq} must satisfy $F(\Pstar + X, \Ahat, \Bhat) = 0$.

The linear map $\opT \colon X \mapsto X - \Lstar^\top X \Lstar$ has eigenvalues equal to $1 - \lambda_i \lambda_j$, where $\lambda_i$ and $\lambda_j$ are eigenvalues of the closed loop matrix $\Lstar$. Since $\Lstar$ is a stable matrix, the linear map $\opT$ must be invertible. Now, we define the operator
\begin{align*}
  \opPhi(X) &= \opT^{-1} \left(F(\Pstar + X, \Astar, \Bstar) - F(\Pstar + X, \Ahat, \Bhat) - \opH(X)\right).
\end{align*}
Then, solving for $X$ in Equation~\ref{eq:fixed_point_eq} is equivalent to finding $X$
\propchange{satisfying $\Pstar + X \succeq 0$}
such that $X = \opPhi(X)$. Hence, $\opPhi$ has a unique symmetric fixed point $X$ such that $\Pstar + X \succeq 0$ and that is $X = \Delta_P$.

Now, we consider the set
%
\begin{align*}
\calS_\nu := \left\{X \colon \norm{X} \leq \nu \text{, } X = X^\top\text{, } \Pstar + X \succeq 0 \right\}
\end{align*}
%
and we show that for an appropriately chosen $\nu$ the operator $\opPhi$ maps $\calS_\nu$ into itself and is also a contraction over the set $\calS_\nu$. If we show these two properties, $\opPhi$ is guaranteed to have a fixed point in the set $\calS_\nu$. However, since $\Delta_P$ is the only possible fixed point of $\opPhi$ in a set $\calS_\nu$ we find $\norm{\Delta_P} \leq \nu$.

We denote $\Delta_A = \Ahat - \Astar$, $\Delta_B = \Bhat - \Bstar$, and $\Delta_S = \Shat - \Sstar$. By assumption we have $\norm{\Delta_A} \leq \varepsilon$ and $\norm{\Delta_B} \leq \varepsilon$. Then, $\norm{\Delta_S} \leq 3 \norm{\Bstar} \norm{R^{-1}}\varepsilon$ because  $\varepsilon \leq \norm{\Bstar}$. The next lemma allows us to complete the argument. Its proof is deferred to Appendix~\ref{app:operator}.

\begin{mylemma}
  \label{lem:operator}
  Suppose the matrices $X$, $X_1$, $X_2$ belong to $\calS_\nu$, with $\nu \leq \min \{ 1, \norm{\Sstar}^{-1}\}$. Furthermore, we assume that $\norm{\Delta_A} \leq \varepsilon$ and $\norm{\Delta_B} \leq \varepsilon$ for $\varepsilon$ such that $\varepsilon \leq \min \{1, \norm{\Bstar} \}$.
  Then
  \begin{align*}
    \norm{\opPhi(X)} &\leq 3 \frac{\transient{\Lstar}{\gamma}^2}{1 - \gamma^2} \left[\norm{\Lstar}^2 \norm{\Sstar} \nu^2 +  \varepsilon \norm{\Astar}_+^2 \norm{\Pstar}^2_+ \norm{\Bstar}_+ \norm{R^{-1}}_+  \right],\\
    \norm{\opPhi(X_1) - \opPhi(X_2)} &\leq 12 \frac{\transient{\Lstar}{\gamma}^2}{1 - \gamma^2} \left[ \norm{\Lstar}^2 \norm{\Sstar} \nu + \varepsilon \norm{\Astar}_+^2 \norm{\Pstar}_+ \norm{\Bstar}_+ \norm{R^{-1}}_+  \right] \norm{X_1 - X_2}.
  \end{align*}
\end{mylemma}

Now, we see that when
\begin{align*}
\nu \leq \frac{1 - \gamma^2}{48 \transient{\Lstar}{\gamma}^2 \norm{\Lstar}^2 \norm{\Sstar}} \; \text{ and }\; \varepsilon \leq \frac{1 - \gamma^2}{48 \transient{\Lstar}{\gamma}^2} \norm{\Astar}_+^{-2} \norm{\Pstar}^{-1}_+ \norm{\Bstar}^{-1}_+ \norm{R^{-1}}^{-1}_+,
\end{align*}
the operator $\opPhi$ satisfies $\norm{\opPhi(X_1) - \opPhi(X_2)} \leq \frac{1}{2}\norm{X_1 - X_2}$ for all $X_1$ and $X_2$ in $\calS_\nu$. Moreover, \propchange{under the same conditions (delete what follows)}
\begin{align}
  \label{eq:conds}
\nu \leq \frac{1 - \gamma^2}{48 \transient{\Lstar}{\gamma}^2 \norm{\Lstar}^2 \norm{\Sstar}} \; \text{ and }\; \varepsilon \leq \nu \frac{1 - \gamma^2}{48 \transient{\Lstar}{\gamma}^2} \norm{\Astar}_+^{-2} \norm{\Pstar}^{-2}_+ \norm{\Bstar}^{-1}_+ \norm{R^{-1}}^{-1}_+,
\end{align}
we have $\norm{\opPhi(X)} \leq \nu$ for all $X\in \calS_\nu$.
\propchange{Do you also need to show that $\Pstar + \opPhi(X) \succeq 0$?}
Then, when conditions \eqref{eq:conds} are satisfied we know that $\opPhi$ maps $\calS_\nu$ into itself and is a contraction over $\calS_\nu$. Therefore, $\opPhi$ has a fixed point in $\calS_\nu$ since $\calS_\nu$ is a closed set. However, we already argued that the unique fixed point of $\opPhi$ is $\Delta_P$. Therefore, $\Delta_P \in \calS_\nu$  and $\norm{\Delta_P} \leq \nu$. Proposition \ref{prop:93} follows because \eqref{eq:conds} are satisfied by assumption.


==> proof_controller.tex <==

\subsection{The nominal controller stabilizes the true system}
\label{sec:controller}

In this section we leverage Proposition~\ref{prop:lipschitz_dare} in order to upper bound the mismatch between the nominal controller and the optimal controller, i.e. to upper bound $\norm{\Khat - \Kstar}$. As a consequence we show that $\Astar + \Bstar \Khat$ is a stable matrix and upper bound its stability radius.

The next two optimization results are helpful in proving $\norm{\Khat - \Kstar}$ is small.

\begin{mylemma}
  \label{lem:strongly_convex_min_perturb}
  Let $f_1, f_2$ be two $\mu$-strongly convex twice differentiable
  functions.  Let $\vecx_1 = \arg\min_\vecx f_1(\vecx)$ and
  $\vecx_2 = \arg\min_\vecx f_2(\vecx)$.  Suppose  $\norm{ \nabla f_1(\vecx_2)} \leq \varepsilon$, then
  $  \norm{\vecx_1 - \vecx_2} \leq \frac{\varepsilon}{\mu}$.
\end{mylemma}
\begin{proof}
  Taylor expanding $\nabla f_1$, we have:
  \begin{align*}
    \nabla f_1(\vecx_2) = \nabla f_1(\vecx_1) + \nabla^2 f_1(\tilde{\vecx}) (\vecx_2 - \vecx_1) = \nabla^2 f_1(\tilde{\vecx}) (\vecx_2 - \vecx_1) \:.
  \end{align*}
  for $\tilde{\vecx} = t \vecx_1 + (1-t) \vecx_2$ with some $t \in [0, 1]$.
  Therefore:
  \begin{align*}
    \mu \norm{\vecx_1 - \vecx_2} \leq \norm{\nabla^2 f_1(\tilde{\vecx}) (\vecx_2 - \vecx_1)} = \norm{\nabla f_1(\vecx_2)} \leq \varepsilon \:.
  \end{align*}
\end{proof}

\begin{mylemma}
  \label{lem:K_perturb_bound}
  Define $f_i(\vecu; \vecx) = \frac{1}{2} \vecu^\T R \vecu + \frac{1}{2}(A_i \vecx + B_i \vecu)^\T
  P_i (A_i \vecx + B_i \vecu)$ for $i=1, 2$, with $R$, $P_1$, and $P_2$  positive definite matrices.  Let $K_i$ be the unique matrix such that
  $\vecu_i := \arg\min_{\vecu} f_i(\vecu; \vecx) =  K_i \vecx$ for any vector $\vecx$. Also, denote $\Gamma := 1 + \max\{\norm{A_1},\norm{B_1},\norm{P_1}, \norm{K_1} \}$. Suppose there exists $\varepsilon$ such that $0 \leq \varepsilon < 1$ and $\norm{A_1-A_2} \leq \varepsilon$, $\norm{B_1-B_2} \leq \varepsilon$, and $\norm{P_1-P_2}  \leq \varepsilon$. Then, we have
  \begin{align*}
    \norm{K_1 - K_2} \leq \frac{7 \varepsilon \Gamma^3 }{\smin(R)} \:.
  \end{align*}
\end{mylemma}
\begin{proof}
  We first compute the gradient $\nabla f_i(\vecu; \vecx)$ with respect to $\vecu$:
  \begin{align*}
    \nabla f_i(\vecu; \vecx) = (B_i^\T P_i B_i + R) \vecu + B_i^\T P_i A_i \vecx \:.
  \end{align*}
  Now, we observe that:
  \begin{align*}
    \norm{B_1^\T P_1 B_1 - B_2^\T P_2 B_2} &\leq 7 \Gamma^2 \varepsilon \; \text{ and } \; \norm{B_1^\T P_1 A_1 - B_2^\T P_2 A_2} = 7\Gamma^2 \varepsilon.
  \end{align*}
  Hence, for any vector $\vecx$ with $\norm{\vecx} \leq 1$, we have
  \begin{align*}
    \norm{ \nabla f_1(\vecu; \vecx) - \nabla f_2(\vecu; \vecx) } &\leq 7 \Gamma^2 \varepsilon (\norm{\vecu} + 1).
  \end{align*}
  We can bound $\norm{\vecu_1} \leq \norm{K_1}\norm{\vecx} \leq \norm{K_1}$. Then, from Lemma~\ref{lem:strongly_convex_min_perturb} we obtain
  \begin{align*}
    \smin(R)\norm{(K_1-K_2)\vecx} = \smin(R)\norm{\vecu_1 - \vecu_2} &\leq 7\Gamma^3 \varepsilon.
  \end{align*}
\end{proof}

Recall that  $\Gamma_\star := 1 + \max\{ \norm{\Astar}, \norm{\Bstar}, \norm{\Pstar}, \norm{\Kstar}\}$. Now, we upper bound $\norm{\Khat - \Kstar}$.

\begin{myprop}
  \label{prop:stability_perturb}
  Let $\rho > \rho(\Astar)$ and let $\varepsilon > 0$ such that
  that $\norm{\Ahat - \Astar} \leq \varepsilon$ and $\norm{\Bhat - \Bstar} \leq \varepsilon$. We denote $\beta := \max\{1, \varepsilon \tau(\Astar, \rho) + \rho \}$. Then, under Assumptions~\ref{ass:controllable} and \ref{ass:strg_cvx} we have
  \begin{align}
    \label{eq:controller_perturb}
    \norm{\Khat - \Kstar} \leq \Ocal(1)\, \varepsilon \, \ell^{\frac{5}{2}} \transient{\Astar}{\rho}^3  \beta^{2(\ell - 1)} \Gamma_\star^6  \left( 1 + \frac{1}{\lbsmin} \right) \frac{ \max \{ \norm{Q}, \norm{R} \} }{\min\{ \smin(R) , \underline{\sigma}(Q)\}} \,.
  \end{align}
  whenever $\varepsilon$ is small enough to ensure the right hand side is smaller than one.
  Let $\gamma$ be a real number such that $\rho(\Astar + \Bstar \Kstar) < \gamma < 1$. Then, if $\varepsilon$ is small enough so that the right hand side of \eqref{eq:controller_perturb} is smaller than $\frac{1 - \gamma}{2 \transient{\Astar + \Bstar \Kstar}{ \gamma}}$, we have
  \begin{align*}
    \tau \left(\Astar + \Bstar \Khat, \frac{1 + \gamma}{2} \right) \leq \transient{\Astar + \Bstar \Kstar}{ \gamma}.
  \end{align*}
\end{myprop}
\begin{proof}
 All the conditions of Proposition~\ref{prop:lipschitz_dare} hold. Therefore, we have
 \begin{align*}
     \|\widehat{P} - \Pstar \|  \leq 32 \, \varepsilon \, \ell^{\frac{5}{2}} \transient{\Astar}{\rho}^3  \beta^{2(\ell - 1)}  \Gamma_\star^3 \left( 1 + \frac{1}{\lbsmin} \right)  \frac{\max \{\|Q\| ,  \|R\| \} }{\min \{ 1, \underline{\sigma}(Q) \} }.
  \end{align*}
  Then, by applying Lemma~\ref{lem:K_perturb_bound} and by the assumption $\smin(R) \geq 1$ we find
  \begin{align*}
    \norm{\Khat - K_\star} \leq 224  \, \varepsilon \, \ell^{\frac{5}{2}} \transient{\Astar}{\rho}^3  \beta^{2(\ell - 1)}  \Gamma_\star^6 \left( 1 + \frac{1}{\lbsmin} \right)  \frac{\max \{\|Q\| ,  \|R\| \} }{\min \{ 1, \underline{\sigma}(Q) \} }.
  \end{align*}

Finally, when $\varepsilon$ is small enough so that the right hand side of \eqref{eq:controller_perturb} is smaller or equal than $\frac{1 - \gamma}{2 \transient{\Astar + \Bstar \Kstar}{ \gamma}}$,  we can apply  Lemma~\ref{lem:lipschitz_matrix_powers} to guarantee that  $\norm{(\Astar + \Bstar \Khat)^k} \leq \transient{\Astar + \Bstar \Kstar}{ \gamma} \left(\frac{1 + \gamma}{2}\right)^k$ for all $k \geq 0$.
\end{proof}


==> proof_main.tex <==


\section{Proof of  Theorem~\ref{thm:meta}}
\label{sec:proof_main}

In this section we prove our meta theorem; we show how an upper bound $\norm{\Phat - \Pstar} \leq f(\varepsilon)$ can be used to quantify the mismatch between the performance of the the nominal controller and the optimal controller. First, we upper bound $\norm{\Khat - \Kstar}$ and offer a condition on this mismatch size so that  $\Astar + \Bstar \Khat$ is a stable matrix. 
%
The next two optimization results are helpful in proving $\norm{\Khat - \Kstar}$ is small.
%
\begin{mylemma}
  \label{lem:strongly_convex_min_perturb}
  Let $f_1, f_2$ be two $\mu$-strongly convex twice differentiable
  functions.  Let $\vecx_1 = \arg\min_\vecx f_1(\vecx)$ and
  $\vecx_2 = \arg\min_\vecx f_2(\vecx)$.  Suppose  $\norm{ \nabla f_1(\vecx_2)} \leq \varepsilon$, then
  $  \norm{\vecx_1 - \vecx_2} \leq \frac{\varepsilon}{\mu}$.
\end{mylemma}
\begin{proof}
  Taylor expanding $\nabla f_1$, we have:
  \begin{align*}
    \nabla f_1(\vecx_2) = \nabla f_1(\vecx_1) + \nabla^2 f_1(\tilde{\vecx}) (\vecx_2 - \vecx_1) = \nabla^2 f_1(\tilde{\vecx}) (\vecx_2 - \vecx_1) \:.
  \end{align*}
  for $\tilde{\vecx} = t \vecx_1 + (1-t) \vecx_2$ with some $t \in [0, 1]$.
  Therefore:
  \begin{align*}
    \mu \norm{\vecx_1 - \vecx_2} \leq \norm{\nabla^2 f_1(\tilde{\vecx}) (\vecx_2 - \vecx_1)} = \norm{\nabla f_1(\vecx_2)} \leq \varepsilon \:.
  \end{align*}
\end{proof}

\begin{mylemma}
  \label{lem:K_perturb_bound}
  Define $f_i(\vecu; \vecx) = \frac{1}{2} \vecu^\T R \vecu + \frac{1}{2}(A_i \vecx + B_i \vecu)^\T
  P_i (A_i \vecx + B_i \vecu)$ for $i=1, 2$, with $R$, $P_1$, and $P_2$  positive definite matrices.  Let $K_i$ be the unique matrix such that
  $\vecu_i := \arg\min_{\vecu} f_i(\vecu; \vecx) =  K_i \vecx$ for any vector $\vecx$. Also, denote $\Gamma := 1 + \max\{\norm{A_1},\norm{B_1},\norm{P_1}, \norm{K_1} \}$. Suppose there exists $\varepsilon$ such that $0 \leq \varepsilon < 1$ and $\norm{A_1-A_2} \leq \varepsilon$, $\norm{B_1-B_2} \leq \varepsilon$, and $\norm{P_1-P_2}  \leq \varepsilon$. Then, we have
  \begin{align*}
    \norm{K_1 - K_2} \leq \frac{7 \varepsilon \Gamma^3 }{\smin(R)} \:.
  \end{align*}
\end{mylemma}
\begin{proof}
  We first compute the gradient $\nabla f_i(\vecu; \vecx)$ with respect to $\vecu$:
  \begin{align*}
    \nabla f_i(\vecu; \vecx) = (B_i^\T P_i B_i + R) \vecu + B_i^\T P_i A_i \vecx \:.
  \end{align*}
  Now, we observe that:
  \begin{align*}
    \norm{B_1^\T P_1 B_1 - B_2^\T P_2 B_2} &\leq 7 \Gamma^2 \varepsilon \; \text{ and } \; \norm{B_1^\T P_1 A_1 - B_2^\T P_2 A_2} = 7\Gamma^2 \varepsilon.
  \end{align*}
  Hence, for any vector $\vecx$ with $\norm{\vecx} \leq 1$, we have
  \begin{align*}
    \norm{ \nabla f_1(\vecu; \vecx) - \nabla f_2(\vecu; \vecx) } &\leq 7 \Gamma^2 \varepsilon (\norm{\vecu} + 1).
  \end{align*}
  We can bound $\norm{\vecu_1} \leq \norm{K_1}\norm{\vecx} \leq \norm{K_1}$. Then, from Lemma~\ref{lem:strongly_convex_min_perturb} we obtain
  \begin{align*}
    \smin(R)\norm{(K_1-K_2)\vecx} = \smin(R)\norm{\vecu_1 - \vecu_2} &\leq 7\Gamma^3 \varepsilon.
  \end{align*}
\end{proof}

Recall that  $\Gamma_\star := 1 + \max\{ \norm{\Astar}, \norm{\Bstar}, \norm{\Pstar}, \norm{\Kstar}\}$. Now, we upper bound $\norm{\Khat - \Kstar}$.

\begin{myprop}
  \label{prop:stability_perturb}
  Let $\varepsilon > 0$ such
  that $\norm{\Ahat - \Astar} \leq \varepsilon$ and $\norm{\Bhat - \Bstar} \leq \varepsilon$. Also, let $\norm{\Phat - \Pstar} \leq f(\varepsilon)$ for some function $f$ such that $f(\varepsilon) \geq \varepsilon$. Then, under Assumption~\ref{ass:strg_cvx} we have
  \begin{align}
    \label{eq:controller_perturb}
    \norm{\Khat - \Kstar} \leq 7 \Gamma_\star^3 \, f(\varepsilon) .
  \end{align}
Let $\gamma$ be a real number such that $\rho(\Lstar) < \gamma < 1$. Then, if $f(\varepsilon)$ is small enough so that the right hand side of \eqref{eq:controller_perturb} is smaller than $\frac{1 - \gamma}{2 \transient{\Lstar}{ \gamma}}$, we have
  \begin{align*}
    \tau \left(\Astar + \Bstar K, \frac{1 + \gamma}{2} \right) \leq \transient{\Lstar}{ \gamma}.
  \end{align*}
\end{myprop}
\begin{proof}
 By our assumptions  $\norm{\Ahat - \Astar}$, $\norm{\Bhat - \Bstar}$, and $\norm{\Phat - \Pstar}$ are smaller than $f(\varepsilon)$, and $\smin(R) \geq 1$.  Then, Lemma~\ref{lem:K_perturb_bound} ensures that
  \begin{align*}
    \norm{\Khat - K_\star} \leq 7  \Gamma_\star^3  \, f(\varepsilon).
  \end{align*}

Finally, when $\varepsilon$ is small enough so that the right hand side of \eqref{eq:controller_perturb} is smaller or equal than $\frac{1 - \gamma}{2 \transient{\Astar + \Bstar \Kstar}{ \gamma}}$,  we can apply  Lemma~\ref{lem:lipschitz_matrix_powers}, presented in Section~\ref{sec:perturb}, to guarantee that  $\norm{(\Astar + \Bstar \Khat)^k} \leq \transient{\Astar + \Bstar \Kstar}{ \gamma} \left(\frac{1 + \gamma}{2}\right)^k$ for all $k \geq 0$.
\end{proof}

In order to finish the proof of Theorem~\ref{thm:meta} we need to quantify the suboptimality gap $\Jhat - J_\star$ in terms of the controller mismatch $\Khat - \Kstar$.
%
For a stable matrix $L$ and a symmetric matrix $M$, we let $\dlyap(L, M)$ denote the solution $X$ to the Lyapunov equation $L^\top X L - X + M = 0$. The following lemma offers a useful second order expansion of the average LQR cost.

\begin{mylemma}[Lemma 12 of \citet{Fazel18}]
\label{lem:second_order_lqr_perturbation}
Let $K$ be an arbitrary static linear controller that stabilizes $(\Astar, \Bstar)$. Denote $\Sigma(K) := \dlyap((\Astar + \Bstar K)^\T, \sigma_w^2 I_n)$ the covariance matrix of the stationary distribution of the closed loop system $\Astar + \Bstar K$.
We have that:
\begin{align}
\label{eq:second_order_expansion}
    J(\Astar, \Bstar, K) - J_\star = \Tr(\Sigma(K) (K - K_\star)^\T (R + \Bstar^\T P_\star\Bstar) (K - K_\star)) \:.
\end{align}
\end{mylemma}
%
Now, we have the necessary ingredients to complete the proof of Theorem~\ref{thm:meta}.
  Equation~\ref{eq:second_order_expansion} implies:
\begin{align*}
J(\Astar, \Bstar, K) - J_\star &\leq \norm{\Sigma(K)} \norm{R + \Bstar^\T \Pstar \Bstar} \norm{K - K_\star}_F^2 \:.
\end{align*}
Proposition~\ref{prop:stability_perturb} states that $\Khat$ stabilizes the system $(\Astar, \Bstar)$ when the estimation error is small enough. More precisely, under the assumptions of Theorem~\ref{thm:meta}, we have
$\tau \left(\Astar + \Bstar \Khat, \frac{1 + \gamma}{2} \right) \leq \transient{\Lstar}{ \gamma}$.
%
When $\widehat{L} = \Astar + \Bstar \Khat$ is a stable matrix we know that $\Sigma(K) = \sigma^2 \sum_{t \geq 0} (L^\top)^t L^t $. Then, by the triangle inequality we can bound 
\begin{align*}
    \norm{\Sigma(K)} \leq \frac{  \sigma_w^2 \transient{\Lstar}{\gamma}^2}{1-\left(\frac{\gamma + 1}{2}\right)^2} \leq \frac{4  \sigma_w^2 \transient{\Lstar}{\gamma}^2}{1 - \gamma^2}\:.
\end{align*}
Recalling that $\Gamma_\star := 1 + \max\{ \norm{\Astar}, \norm{\Bstar}, \norm{\Pstar}, \norm{\Kstar}\}$, we have $\norm{R + \Bstar^\T \Pstar \Bstar} \leq \Gamma^3$. Then,
\begin{align*}
  J(K) - J_\star &\leq 4 \sigma_w^2 \Gamma^3  \frac{ \transient{\Lstar}{\gamma}^2}{1- \gamma^2} \norm{K - K_\star}_F^2\\
                 &\leq 4 \sigma_w^2 \min \{ \statedim , \inputdim \} \Gamma^3 \frac{ \tau(\Lstar, \gamma)^2}{1- \gamma^2}  \norm{K - K_\star}^2 \\
  &\leq 200 \sigma_w^2 d \Gamma^9 \frac{ \tau(\Lstar, \gamma)^2}{1- \gamma^2} f(\varepsilon)^2,
\end{align*}
where we used Proposition~\ref{prop:stability_perturb} and the assumption on $f(\varepsilon)$. 


==> proof_perturbation_dare.tex <==

\section{Perturbation of the discrete algebraic Riccati equation}
\label{sec:perturb}

\subsection{Proof of Proposition~\ref{prop:93}}
\label{sec:proof_93}

Given parameters $(A,B, Q)$ ($R$ is assumed fixed throughout; $Q$ is assumed positive semidefinite throughout) we denote by $F(X, A, B, Q)$ the matrix expression
\begin{align}
  F(X, A, B, Q) &= X - A^\top X A + A^\top X B (R + B^\top X B)^{-1} B^\top X A - Q \nonumber \\
             &= X - A^\top X\left( I + B R^{-1} B^\top X  \right)^{-1}A - Q \:. \label{eq:riccati_op_short}
\end{align}
Then, solving the Riccati equation associated with $(A, B, Q)$ corresponds to finding the unique positive definite matrix $X$ such that $F(X, A, B, Q) = 0$. We denote by $\Pstar$ the solution of the Riccati equation corresponding to the true system parameters $(\Astar, \Bstar)$ and we denote by $\Phat$ the solution associated with $(\Ahat, \Bhat, \Qh)$. Our goal is to upper bound $\norm{\Phat - \Pstar}$ in terms of $\varepsilon$, where $\varepsilon > 0$ such that $\norm{\Ahat - \Astar} \leq \varepsilon$, $\norm{\Bhat - \Bstar} \leq \varepsilon$, and  $\norm{\Qh - Q_\star} \leq \varepsilon$.

We denote $\Delta_P = \Phat - \Pstar$. The proof strategy goes as follows. Given the identities $F(\Pstar, \Astar, \Bstar, Q_\star) = 0$ and $F(\Phat, \Ahat, \Bhat, \Qh) = 0$ we construct an operator $\opPhi$ such that $\Delta_P$ is its unique fixed point. Then, we show that the fixed point of $\opPhi$ must have small norm when $\varepsilon$ is sufficiently small.

We denote $S_\star = \Bstar R^{-1} \Bstar^\top$ and $\Shat = \Bhat R^{-1} \Bhat^\top$. Also, recall that $L_\star = \Astar + \Bstar \Kstar$. For any matrix $X$ such that $I + \Sstar(\Pstar + X)$ is invertible we have
\begin{align}
  \label{eq:magical}
F(\Pstar + X, \Astar, \Bstar, Q_\star) &= X - L_\star^\top X L_\star + L_\star^\top X \left[I + S_\star (\Pstar + X)\right]^{-1} S_\star X L_\star.
\end{align}
To check this identity one needs to add  $F(\Pstar, \Astar, \Bstar, Q_\star)$, which is equal to zero, to the right hand side of \eqref{eq:magical} and use the identity $(I + \Bstar R^{-1} \Bstar^\top \Pstar)^{-1} \Astar = \Astar + \Bstar \Kstar$. This last identity can be checked by recalling $\Kstar = - (R + \Bstar^\top \Pstar \Bstar)^{-1} \Bstar^\top \Pstar \Astar$ and using the matrix inversion formulat.

To write \eqref{eq:magical} more compactly we define the following two matrix operators
\begin{align*}
\opT(X) = X - L_\star^\top X L_\star \;\text{ and }\; \opH(X) = L_\star^\top X \left(I + S_\star(\Pstar + X)\right)^{-1} S_\star X L_\star.
\end{align*}
Then, Equation~\ref{eq:magical} becomes $F(\Pstar + X, \Astar, \Bstar, Q_\star) = \opT(X) + \opH(X)$.
Since Equation~\ref{eq:magical} is satisfied by any matrix $X$ with $I + S_\star(\Pstar+X)$ invertible, the matrix equation
\begin{align}
  \label{eq:fixed_point_eq}
  F(\Pstar + X, \Astar, \Bstar, Q_\star) - F(\Pstar + X, \Ahat, \Bhat, \Qh) = \opT(X) + \opH(X)
\end{align}
 has a unique symmetric solution $X$ such that $\Pstar + X \succeq 0$.
That solution is $X = \Delta_P$ because any solution of \eqref{eq:fixed_point_eq} must satisfy $F(\Pstar + X, \Ahat, \Bhat, \Qh) = 0$.

The linear map $\opT \colon X \mapsto X - \Lstar^\top X \Lstar$ has eigenvalues equal to $1 - \lambda_i \lambda_j$, where $\lambda_i$ and $\lambda_j$ are eigenvalues of the closed loop matrix $\Lstar$. Since $\Lstar$ is a stable matrix, the linear map $\opT$ must be invertible. Now, we define the operator
\begin{align*}
  \opPhi(X) &= \opT^{-1} \left(F(\Pstar + X, \Astar, \Bstar, Q_\star) - F(\Pstar + X, \Ahat, \Bhat, \Qh) - \opH(X)\right).
\end{align*}
Then, solving for $X$ in Equation~\ref{eq:fixed_point_eq} is equivalent to finding $X$ satisfying $\Pstar + X \succeq 0$ such that $X = \opPhi(X)$. Hence, $\opPhi$ has a unique symmetric fixed point $X$ such that $\Pstar + X \succeq 0$ and that is $X = \Delta_P$. Now, we consider the set
%
\begin{align*}
\calS_\nu := \left\{X \colon \norm{X} \leq \nu \text{, } X = X^\top\text{, } \Pstar + X \succeq 0 \right\}
\end{align*}
%
and we show that for an appropriately chosen $\nu$ the operator $\opPhi$ maps $\calS_\nu$ into itself and is also a contraction over the set $\calS_\nu$. If we show these two properties, $\opPhi$ is guaranteed to have a fixed point in the set $\calS_\nu$. However, since $\Delta_P$ is the only possible fixed point of $\opPhi$ in a set $\calS_\nu$ we find $\norm{\Delta_P} \leq \nu$.

We denote $\Delta_A = \Ahat - \Astar$, $\Delta_B = \Bhat - \Bstar$, $\Delta_Q = \Qh - Q_\star$, and $\Delta_S = \Shat - \Sstar$. By assumption we have $\norm{\Delta_A} \leq \varepsilon$,  $\norm{\Delta_B} \leq \varepsilon$, $\norm{\Delta_Q} \leq \varepsilon$. Then, $\norm{\Delta_S} \leq 3 \norm{\Bstar} \norm{R^{-1}}\varepsilon$ because  $\varepsilon \leq \norm{\Bstar}$. %The next lemma assumes $\Qh = Q_\star$; its proof relies on just algebraic computations which can be extended to the case $\Qh \neq Q_\star$. 
\begin{mylemma}
  \label{lem:operator_93}
  Suppose the matrices $X$, $X_1$, $X_2$ belong to $\calS_\nu$, with $\nu \leq \min \{ 1, \norm{\Sstar}^{-1}\}$. Furthermore, we assume that $\norm{\Delta_A} \leq \varepsilon$, $\norm{\Delta_B} \leq \varepsilon$, and $\norm{\Delta_Q} \leq \varepsilon$ with $\varepsilon \leq \min \{1, \norm{\Bstar} \}$. Finally, let $\smin(\Pstar) \geq 1$. Then
  \begin{align*}
    \norm{\opPhi(X)} &\leq 3 \frac{\transient{\Lstar}{\gamma}^2}{1 - \gamma^2} \left[\norm{\Lstar}^2 \norm{\Sstar} \nu^2 +  \varepsilon \norm{\Astar}_+^2 \norm{\Pstar}^2_+ \norm{\Bstar}_+ \norm{R^{-1}}_+  \right],\\
    \norm{\opPhi(X_1) - \opPhi(X_2)} &\leq 32 \frac{\transient{\Lstar}{\gamma}^2}{1 - \gamma^2} \left[ \norm{\Lstar}^2 \norm{\Sstar} \nu + \varepsilon \norm{\Astar}_+^2 \norm{\Pstar}^3_+ \norm{\Bstar}^3_+ \norm{R^{-1}}^2_+  \right] \norm{X_1 - X_2}.
  \end{align*}
\end{mylemma}
The proof of this lemma is defered to Appendix~\ref{app:lem_93}. Now, we choose
\begin{align}
  \label{eq:nu_choice}
  \nu = 6 \, \varepsilon \, \frac{\transient{\Lstar}{ \gamma}^2}{1 - \gamma^2} \norm{\Astar}_+^2 \norm{\Pstar}_+^2\norm{\Bstar}_+ \norm{R^{-1}}_+.
\end{align}
Since $\varepsilon$ is assumed to be small enough, we know
\begin{align*}
\nu  \leq \min \left\{ \frac{1 - \gamma^2}{128 \transient{\Lstar}{\gamma}^2 \norm{\Lstar}^2 \norm{\Sstar}}, \norm{\Sstar}^{-1},  \frac{1}{2} \right\}.
\end{align*}
Then, the operator $\opPhi$ satisfies $\norm{\opPhi(X_1) - \opPhi(X_2)} \leq \frac{1}{2}\norm{X_1 - X_2}$ for all $X_1$ and $X_2$ in $\calS_\nu$. Moreover, we have $\norm{\opPhi(X)} \leq \nu$ for all $X\in \calS_\nu$. Since $\nu \leq \smin(\Pstar)$, we know that $\Pstar + \opPhi(X) \succeq 0$ 

Therefore, $\opPhi$ maps $\calS_\nu$ into itself and is a contraction over $\calS_\nu$. Hence, $\opPhi$ has a fixed point in $\calS_\nu$ since $\calS_\nu$ is a closed set. However, we already argued that the unique fixed point of $\opPhi$ is $\Delta_P$. Therefore, $\Delta_P \in \calS_\nu$  and $\norm{\Delta_P} \leq \nu$. Proposition \ref{prop:93} is now proven. 


\subsection{Proof of Proposition~\ref{prop:lipschitz_dare}}
\label{sec:proof_dare}

Since both noisy and noiseless LQR have the same associated Riccati equation and the same optimal controller, we can focus on the noiseless case in this section. Namely, noiseless LQR takes the form
\begin{align*}
  \min_{\vecu} \sum_{t = 0}^\infty \vecx_t^\top Q \vecx_t + \vecu_t^\top R \vecu_t \; \text{, where } \; \vecx_{t + 1} = \Astar \vecx_t + \Bstar \vecu_t,
\end{align*}
for a given initial state $\vecx_0$. Then, we know that the cost achieved by the optimal controller
when the system is initialized at $\vecx_0$ is equal to $\vecx_0^\top \Pstar \vecx_0$.

We denote by
$J(A, B, \vecx_0, \{\vecu_t \}_{t \geq 0})$ the cost achieved on a
linear system $(A, B)$ initialized at $\vecx_0$ by the input sequence $\{ \vecu_t\}_{t \geq 0}$. When the input sequence is
given by a time invariant linear gain matrix $K$ we slightly abuse notation and denote the cost by $J(A, B, \vecx_0, K)$. In this case, $J(A, B, \vecx_0, K)= \vecx_0^\top P \vecx_0$, where $P$ is the solution to the associated Riccati equation.

Now, let $\vecx_0$ be an arbitrary unit state vector in $\R^\statedim$. Then,
\begin{align*}
  \vecx_0^\top \Phat \vecx_0 - \vecx_0^\top \Pstar \vecx_0 &= J(\Ahat, \Bhat, \vecx_0, \Khat) - J(\Astar, \Bstar, \vecx_0, \Kstar) \\
                                                           &\leq J(\Ahat, \Bhat, \vecx_0, \{ \widehat{\vecu}_t\}_{t \geq 0}) - J(\Astar, \Bstar, \vecx_0, \Kstar)
\end{align*}
for any sequence of inputs $\{\widehat{\vecu}_{t} \}_{t \geq 0}$. We denote by $\hat{\vecx}_t$ the states produced by
$\widehat{\vecu}_t$ on the system $(\Ahat, \Bhat)$ and by $\vecx_t$
and $\vecu_t$ the states and actions obtained on the system
$(\Astar, \Bstar)$ when the optimal controller $\vecu_t = \Kstar \vecx_t$ is used. To prove
Proposition~\ref{prop:lipschitz_dare} we choose a sequence of actions
$ \{ \widehat{\vecu}_t\}_{t \geq 0}$ such that $ J(\Ahat, \Bhat, \vecx_0, \{ \widehat{\vecu}_t\}_{t \geq 0}) \approx
J(\Astar, \Bstar, \vecx_0, \Kstar)$.

For any sequence of inputs $\{\widehat{\vecu}_{t}\}_{t \geq 0}$ such that the series defining the cost $J(\Ahat, \Bhat, \vecx_0, \{ \widehat{\vecu}_t\}_{t \geq 0})$ is
absolutely convergent, we can write
\begin{align}
  \label{eq:block_series}
  J(\Ahat, \Bhat, \vecx_0, \Khat) - J(\Astar, \Bstar, \vecx_0, \Kstar) &= \sum_{j = 0}^{\infty} \sum_{i = 0}^{\ell - 1} \left[ \widehat{\vecx}_{\ell j + i}^\top Q \widehat{\vecx}_{\ell j + i} - \vecx_{\ell j + i}^\top Q  \vecx_{\ell j + i} \right]\\
  \nonumber
                                                                       &\quad + \sum_{j = 0}^{\infty} \sum_{i = 0}^{\ell - 1} \left[  \widehat{\vecu}_{\ell j + i}^\top R \widehat{\vecu}_{\ell j + i}  -  \vecu_{\ell j + i}^\top R   \vecu_{\ell j + i} \right].
\end{align}
Then, the key idea is to choose a sequence of inputs
$\{\widehat{\vecu}_{t} \}_{t \geq 0}$ such that the system
$(\Ahat, \Bhat)$ tracks the system $(\Astar, \Bstar, \Kstar)$, i.e.,
$\widehat{\vecx}_{\ell j} = \vecx_{\ell j}$ for any $j \geq 0$ (
$\widehat{\vecx}_0 = \vecx_0$ because both systems are initialized at
the same state). This can be done because $(\Ahat, \Bhat)$ is $(\ell, \tau / 2)$-controllable when $(\Astar, \Bstar)$ is $(\ell, \tau)$-controllable and the estimation error is sufficiently small, as shown in Lemma~\ref{lem:controllable_perturb}.
First, we present a result that quantifies the effect of matrix perturbations on powers of matrices.

\begin{mylemma}
  \label{lem:lipschitz_matrix_powers}
  Let $M$ be an arbitrary matrix in $\R^{\statedim \times \statedim}$
  and let $\rho \geq \rho(M)$. Then, for all
  $k \geq 1$ and real matrices $\Delta$ of appropriate dimensions we have

\begin{align*}
   \norm{(M + \Delta)^k} &\leq \transient{M}{\rho} ( \transient{M}{\rho} \norm{\Delta} + \rho)^{k},\\
  \norm{(M + \Delta)^k - M^k} &\leq k \, \transient{M}{\rho}^2 ( \transient{M}{\rho} \norm{\Delta} + \rho)^{k - 1} \norm{\Delta}.
\end{align*}
Recall that $\transient{M}{\rho}$ is defined in Equation~\ref{eq:transient}.
\end{mylemma}
The proof is deferred to Appendix~\ref{app:proof_lemma_matrix_perturb}.
Lemma~\ref{lem:lipschitz_matrix_powers} quantifies the effect of a perturbation $\Delta$,
applied to a matrix $M$ on the spectral radius of $M + \Delta$. We are interested
in quantifying the sizes of these perturbations for all $k = 1, 2, \ldots, \ell$. Depending on $\norm{\Delta}$, $M$, and $\rho$ the sum $\tau(M, \rho) \norm{\Delta} + \rho$ can either be greater than one or smaller than one. For notational
simplicity, in the rest of the proof we denote $\beta = \max\{1, \varepsilon  \transient{\Astar}{\rho}  + \rho\}$. Then,
we have $\norm{(\Astar + \Delta)^k} \leq \transient{\Astar}{\rho} \beta^{\ell - 1}$ and $\norm{(\Astar + \Delta)^k - \Astar^k} \leq \ell \transient{\Astar}{\rho}^2 \beta^{\ell - 1} \varepsilon$ for all $k \leq \ell - 1$ and all real matrices $\Delta$ with $\norm{\Delta} \leq \varepsilon$.

We denote $C_\ell = \begin{bmatrix}
\Bstar & \Astar \Bstar & \ldots & \Astar^{\ell - 1} \Bstar
\end{bmatrix} $ and $\widehat{\Ccal}_\ell = \begin{bmatrix} \Bhat & \Ahat\Bhat & \ldots &
  \Ahat^{\ell - 1}\Bhat \end{bmatrix}$. Before presenting the next result
we recall that for any block matrix $M$ with blocks $M_{i,j}$ we have
$  \|M\|^2 \leq  \sum_{i,j} \|M_{i,j}\|^2$.
%
The next lemma gives us control over the smallest positive singular value of the controllability matrix $\widehat{\Ccal}_\ell$ in terms of the corresponding value for $\Ccal_\ell$.

\begin{mylemma}
  \label{lem:controllable_perturb}
  Suppose the linear $(\Astar, \Bstar)$ is $(\ell, \lbsmin)$-controllable and let $\rho$ be a real number such that $\rho \geq \rho(\Astar)$. Then, if
  $\| \Ahat - \Astar \| \leq \varepsilon$ and
  $\| \Bhat - \Bstar \| \leq \varepsilon$,
  we have
  \begin{align*}
    \underline{\sigma}(\widehat{C}_\ell) \geq \tau - 3 \varepsilon \ell^{\frac{3}{2}} \transient{\Astar}{\rho}^2  \max\{1, \transient{\Astar}{\rho} \norm{\Delta} + \rho\}^{\ell - 1} \left( \norm{\Bstar} + 1 \right). \end{align*}
\end{mylemma}
The proof is deferred to Appendix~\ref{app:proof_controllable_perturb}.
%
Lemma~\ref{lem:controllable_perturb} tells us that
by the assumption made in Proposition~\ref{prop:lipschitz_dare} on $\varepsilon$, we have
$\underline{\sigma}(\widehat{\Ccal}_\ell) \geq
\frac{\tau_\ell}{2}$. Hence, we know that for any $\vecx_0\in \RR^\statedim$ and $\vecu_0, \vecu_1, \ldots, \vecu_{\ell - 1}\in \RR^\inputdim$, there
exist $\widehat{\vecu}_0, \widehat{\vecu}_1, \ldots, \widehat{\vecu}_{\ell -
  1} \in \RR^\inputdim$ such that
\begin{align}
  \label{eq:matching_states}
  \Astar^{\ell} \vecx_0 + \sum_{i = 0}^{\ell - 1} \Astar^i \Bstar\vecu_{\ell - 1 - i} = \Ahat^{\ell} \vecx_0 + \sum_{i = 0}^{\ell - 1}\Ahat^i\Bhat\widehat{\vecu}_{\ell - 1 - i}
\end{align}
because the system $(\Ahat, \Bhat)$ is controllable. This equation implies that $\widehat{\vecx}_\ell = \vecx_\ell$.
% In order to avoid cumbersome notation we think inductively and consider each state $\vecx_{\ell j}$
%as the new initial vector $\vecx_0$ in Equation \eqref{eq:block_series}.

We denote the concatenation of $\vecu_i$, for $i$ from $0$ to
$\ell - 1$ by $\vecu^{(\ell)}$. We define $\widehat{\vecu}^{(\ell)}$ analogously. Therefore, Equation~\eqref{eq:matching_states} can be
rewritten as
\begin{align}
  \label{eq:tracking}
  \left( \Astar^\ell - \widehat{A}^\ell  \right) \vecx_0 + \left(\mathcal{C}_\ell - \widehat{\mathcal{C}}_\ell \right) \vecu^{(\ell)} = \widehat{\mathcal{C}}_\ell (\widehat{\vecu}^{(\ell)} - \vecu^{(\ell)}).
\end{align}
%
Recall that $\beta = \max\{1, \transient{\Astar}{\rho} \norm{\Delta} + \rho\}$.
Combining Lemma~\ref{lem:lipschitz_matrix_powers} and the upper bound on operator norms of block matrices we find $\| \widehat{\Ccal}_\ell - \Ccal_\ell \| \leq \varepsilon \ell^{\frac{3}{2}} \transient{\Astar}{ \rho}^2 \beta^{\ell - 1} \left( \| \Bstar \| + 1 \right)$.

%
We are free to choose $\widehat{\vecu}^{(\ell)}$ anyway we wish as long as Equation~\eqref{eq:tracking} is true. Therefore, we can choose $\widehat{\vecu}^{(\ell)}$
such that $\widehat{\vecu}^{(\ell)} - \vecu^{(\ell)}$ is perpendicular to the nullspace of $\widehat{\Ccal}_\ell$. Then,
\begin{align*}
  \frac{\tau_\ell}{2} \|\widehat{\vecu}^{(\ell)} - \vecu^{(\ell)} \| &\leq \| \widehat{\Ccal}_\ell(\widehat{\vecu}^{(\ell)} - \vecu^{(\ell)} ) \| \leq \varepsilon \ell \transient{\Astar}{ \rho}^2 \beta^{\ell - 1} \| \vecx_0\| + \|\widehat{\Ccal}_\ell - \Ccal_\ell\| \| \vecu^{(\ell)}\| \\
 &\leq \varepsilon \ell \transient{\Astar}{ \rho}^2 \beta^{\ell - 1} \| \vecx_0\|  + \varepsilon \ell^{\frac{3}{2}} \transient{\Astar}{ \rho}^2 \beta^{\ell - 1} \left(\|\Bstar \| + 1 \right) \| \vecu^{(\ell)}\|.
\end{align*}
%
Hence,
\begin{align}
    \nonumber
  \|\widehat{\vecu}^{(\ell)} - \vecu^{(\ell)} \|
  &\leq \frac{2 \varepsilon \ell^{\frac{3}{2}}}{\tau_\ell} \transient{\Astar}{ \rho}^2 \beta^{\ell - 1} (\| \Bstar \| + 1) \left( \| \vecx_0 \| + \| \vecu^{(\ell)} \| \right)\\
  \label{eq:u_bound}
  &=: \eta \left( \| \vecx_0 \| + \| \vecu^{(\ell)} \| \right) \:.
\end{align}
%
Let us consider the block Toeplitz matrix
\begin{align*}
  \Tcal_\ell = \begin{bmatrix}
    0 & 0 & 0 & \ldots & 0\\
    \Bstar & 0 & 0 & \cdots & 0\\
    \Astar \Bstar & \Bstar & 0 & \cdots & 0 \\
    \vdots & \cdots & \cdots & \cdots & \cdots  \\
    \Astar^{\ell - 2} \Bstar & \Astar^{\ell - 3} \Bstar & \cdots & \Bstar & 0
  \end{bmatrix}.
\end{align*}
From Lemma~\ref{lem:lipschitz_matrix_powers} and the upper bound on operator norms of block matrices we have
$\|\Tcal_\ell - \widehat{\Tcal}_\ell\| \leq \varepsilon \ell^2 \transient{\Astar}{\rho}^2 \beta^{\ell - 2}(\|\Bstar \| + 1)$.
% where $\beta =  \max\{1, \transient{\Astar}{\rho} \norm{\Delta} + \rho\}$.
Let $\vecx^{(\ell)}$ be the concatenation of the vectors $\vecx_0$, $\vecx_1$, \ldots, $\vecx_{\ell - 1}$. Then,
\begin{align*}
  \vecx^{(\ell)} = \Tcal_\ell \vecu^{(\ell)} + \begin{bmatrix}
    I_\statedim \\
    \Astar\\
    \vdots\\
    A^{\ell - 1}
  \end{bmatrix}
  \vecx_0.
\end{align*}
%
Hence,
\begin{align}
  \nonumber
  \| \vecx^{(\ell)}  -  \widehat{\vecx}^{(\ell)} \| &\leq \| \Tcal_\ell \vecu^{(\ell)}  - \widehat{\Tcal}_\ell \widehat{\vecu}^{(\ell)}  \| + \varepsilon \ell^{\frac{3}{2}} \transient{\Astar}{\rho}^2 \beta^{\ell - 2} \| \vecx_0 \| \\
    \nonumber
                                                    &\leq \| \Tcal_\ell \vecu^{(\ell)}  - \widehat{\Tcal}_\ell \vecu^{(\ell)}  \| + \| \widehat{\Tcal}_\ell \vecu^{(\ell)}  - \widehat{\Tcal}_\ell \widehat{\vecu}^{(\ell)}  \| +  \varepsilon \ell^{\frac{3}{2}}  \transient{\Astar}{ \rho}^2 \beta^{\ell - 2} \| \vecx_0 \| \\
    \nonumber
                                                    &\leq \| \Tcal_\ell  - \widehat{\Tcal}_\ell \| \| \vecu^{(\ell)}  \| + \| \widehat{\Tcal}_\ell\| \| \vecu^{(\ell)}  - \widehat{\vecu}^{(\ell)}  \| +  \varepsilon \ell^{\frac{3}{2}}  \transient{\Astar}{\rho}^2 \beta^{\ell - 2} \| \vecx_0 \|  \\
    \nonumber
                                                    &\leq  \varepsilon \ell^2 \transient{\Astar}{\rho}^2 \beta^{\ell - 2}(\|\Bstar \| + 1) \| \vecu^{(\ell)}  \| +  \varepsilon  \ell^{\frac{3}{2}}  \transient{\Astar}{\rho}^2 \beta^{\ell - 2} \| \vecx_0 \|   \\
    \nonumber
                                                    &\quad + \ell \transient{\Astar}{\rho} \beta^{\ell - 2} (\|\Bstar\| + 1) \| \vecu^{(\ell)}  - \widehat{\vecu}^{(\ell)}  \| \\
    \nonumber
                                                    &\leq 2 \varepsilon \ell^{\frac{5}{2}} \transient{\Astar}{\rho}^3 \beta^{2(\ell - 1)} (1 + \tau^{-1}) (\|\Bstar \| + 1)^2  \left[ \| \vecx_0 \| + \|\vecu^{(\ell)}\| \right] \\
  \label{eq:x_bound}
                                                      &=: \mu \left[  \| \vecu^{(\ell)}  \| +  \| \vecx_0 \| \right].
\end{align}
%
In Equations \eqref{eq:u_bound} and \eqref{eq:x_bound} we proved that the inputs and states of the system $(\Ahat, \Bhat)$ are close to the inputs and states of the system $(\Astar, \Bstar)$ from time $0$ to $\ell$. Since the inputs to the system $(\Ahat, \Bhat)$ satisfy Equation~\eqref{eq:tracking}, we know that $\widehat{\vecx}_{\ell j} = \vecx_{\ell j}$ for all $j$. We can repeat the same argument as above, with $\vecx_{\ell j}$ taking the place of $\vecx_0$, to show that the inputs and states of the two systems are close to each other from time $\ell j$ to $\ell (j + 1)$. Let us denote by $\vecx_j^{(\ell)}$ the concatenation of the vectors $\vecx_{\ell j}$, $\vecx_{\ell j + 1}$, \ldots, $\vecx_{\ell j + \ell - 1}$ and let $\vecu_j^{(\ell)}$ be defined analogously. Then,
\begin{align}
  \label{eq:u_j_bound}
  \|\widehat{\vecu}_j^{(\ell)} - \vecu_j^{(\ell)} \| &\leq  \eta \left[ \| \vecu_j^{(\ell)} \| +  \| \vecx_{\ell j} \| \right], \; \text{ and }\;
  \| \widehat{\vecx}_j^{(\ell)}  -  \vecx_j^{(\ell)}    \| \leq \mu \left[\| \vecu_j^{(\ell)}  \| +  \| \vecx_{\ell j} \| \right].
\end{align}
Now, we note that
\begin{align*}
  \vecx_0^\top \Phat \vecx_0 - \vecx_0^\top \Pstar \vecx_0  &\leq \sum_{j = 0}^{\infty} \sum_{i = 0}^{\ell - 1} \left[ \widehat{\vecx}_{\ell j + i}^\top Q \widehat{\vecx}_{\ell j + i} - \vecx_{\ell j + i}^\top Q  \vecx_{\ell j + i} \right]\\
                         &\quad + \sum_{j = 0}^{\infty} \sum_{i = 0}^{\ell - 1} \left[  \widehat{\vecu}_{\ell j + i}^\top R \widehat{\vecu}_{\ell j + i}  -  \vecu_{\ell j + i}^\top R   \vecu_{\ell j + i} \right]\\
                         &\leq \sum_{j = 0}^{\infty} 2 \|Q \| \| \vecx_j^{(\ell)}\| \| \vecx_{j}^{(\ell)}  -  \widehat{\vecx}_{j}^{(\ell)} \| + \|Q\| \| \vecx_{j}^{(\ell)}  -  \widehat{\vecx}_{j}^{(\ell)} \|^2  \\
                         &\quad +  \sum_{j = 0}^{\infty} 2 \|R \| \| \vecu_{j}^{(\ell)}\| \| \vecu_{j}^{(\ell)}  -  \widehat{\vecu}_{j}^{(\ell)} \| + \|R\| \| \vecu_{j}^{(\ell)}  -  \widehat{\vecu}_{j}^{(\ell)} \|^2 \:.
\end{align*}
%
%Now, we use the upper bounds \eqref{eq:u_j_bound} to show that the right hand side is small.
%Since $\vecx_0$ is an arbitrary unit vector, this analysis shows that $\lambda_{\max}\left(\Phat - \Pstar\right)$ is small. Swapping
%the roles of $(\Ahat, \Bhat)$ and $(\Astar, \Bstar)$ gives us that $\lambda_{\max}\left(\Pstar - \Phat\right)$ is also small, yielding the desired conclusion. We defer the details of this argument to Appendix~\ref{app:remainder_proof_perturb}.
%
Now, we use the upper bounds from \eqref{eq:u_j_bound}. We always have $\eta \leq \mu$. Since Proposition~\ref{prop:lipschitz_dare} assumes $\varepsilon$ is  small enough, we also have $\mu \leq 1$. Using these upper bounds, we find
\begin{align*}
  \widehat{J} - J_\star  &\leq \mu \sum_{j = 0}^{\infty} 2 \|Q \| \| \vecx_j^{(\ell)}\| \left[\| \vecu_j^{(\ell)}  \| +  \| \vecx_{\ell j} \| \right] + \|Q\| \left[\| \vecu_j^{(\ell)}  \| +  \| \vecx_{\ell j} \| \right]^2  \\
                         &\quad + \mu \sum_{j = 0}^{\infty} 2 \|R \| \| \vecu_{j}^{(\ell)}\| \left[\| \vecu_j^{(\ell)}  \| +  \| \vecx_{\ell j} \| \right]  + \|R\| \left[\| \vecu_j^{(\ell)}  \| +  \| \vecx_{\ell j} \| \right]^2 \:.
\end{align*}
%
Then, we get $\widehat{J} - J_\star \leq 8 \mu \max\{ \|Q\| , \|R\| \} \sum_{j = 0}^\infty \| \vecx_{j}^{(\ell)}\|^2 + \| \vecu_{j}^{(\ell)}\|^2$ after using the inequalities $(a + b)^2 \leq 2(a^2 + b^2)$ and $2ab \leq a^2 + b^2$.
%
Now, As long as $\norm{\vecx_0} \leq 1$ we have
\begin{align}
  \label{eq:upper_bound_states_series}
  \min \{ \underline{\sigma}(Q) , \underline{\sigma}(R) \} \sum_{j = 0}^\infty  \| \vecx_j^{(\ell)}\|^2 +  \| \vecu_j^{(\ell)}\|^2 \leq \sum_{t = 0}^\infty \vecx_t^\top Q \vecx_t + \vecu_t^\top R \vecu_t =
  \vecx_0^\top \Pstar \vecx_0  \leq \|\Pstar\|.
\end{align}
%
Since the initial state is an arbitrary unit norm vector, our upper bound on $\vecx_0^\top (\Phat - \Pstar) \vecx_0$ becomes
\begin{align}
  \label{eq:j_jhat_2}
  \lambda_{\max} \left(\widehat{P} - \Pstar \right) \leq 16 \varepsilon \ell^{\frac{5}{2}}  \transient{\Astar}{\rho}^3 \beta^{2(\ell - 1)} (1 + \lbsmin^{-1}) ( 1 + \|\Bstar \| )^2 \|P_\star \| \frac{ \max\{ \|Q\|,   \|R\| \} }{ \min \{ \underline{\sigma}(Q) ,  \underline{\sigma}(R) \} }.
\end{align}
%
Now, we can reverse the roles of $(\Ahat, \Bhat)$ and
$(\Astar, \Bstar)$ and repeat the same argument and obtain an upper bound
on $\lambda_{\max}\left(\Pstar - \widehat{P}\right)$ analogous to Equation~\eqref{eq:j_jhat_2},
but which has $\|P_\star\|$ replaced by $\|\widehat{P}\|$ on the right hand side. However,
\eqref{eq:j_jhat_2} implies that $\|\widehat{P}\| \leq \|P_\star \| + 1 \leq 2 \|P_\star \|$ because we assumed that $\varepsilon$ is small enough such that the right hand side of \eqref{eq:j_jhat_2} is less than one, and because $\Pstar \succeq I_\statedim$. The conclusion follows.

We note that the proof can be easily extended to the case when the cost matrix $Q$ is also being perturbed. Moreover, the only essiential step in the argument where we used $Q \succ 0$ is \eqref{eq:upper_bound_states_series}. The goal of \eqref{eq:upper_bound_states_series} is to upper bound  $\sum_{j = 0}^\infty \| \vecx_{j}^{(\ell)}\|^2 + \| \vecu_{j}^{(\ell)}\|^2$. This quantity can be upper bounded even when $Q$ is not positive definite, but the system $(Q^{1/2}, A)$ is observable; which is a necessary requirement for LQR on the parameters $(A,B,Q,R)$ to stabilize the system $(A,B)$. 
